Be Careful What You Smooth For: Label Smoothing Can Be a Privacy Shield but Also a Catalyst for Model Inversion Attacks

Label smoothing -- using softened labels instead of hard ones -- is a widely adopted regularization method for deep learning, showing diverse benefits such as enhanced generalization and calibration. Its implications for preserving model privacy, however, have remained unexplored. To fill this gap, we investigate the impact of label smoothing on model inversion attacks (MIAs), which aim to generate class-representative samples by exploiting the knowledge encoded in a classifier, thereby inferring sensitive information about its training data. Through extensive analyses, we uncover that traditional label smoothing fosters MIAs, thereby increasing a model's privacy leakage. Even more, we reveal that smoothing with negative factors counters this trend, impeding the extraction of class-related information and leading to privacy preservation, beating state-of-the-art defenses. This establishes a practical and powerful novel way for enhancing model resilience against MIAs.

==> sections/C_datasets.tex <==
\section{Datasets}\label{app:dataset}

We split each training dataset into 90\% training data and 10\% test data. The splits are identical for all target and evaluation models. The test data is only used to evaluate the models' prediction accuracy. We further want to point out that neither the StyleGAN2 models nor the attacks have access to the target models' training data. The datasets are only used to evaluate the attack results after the attacks were finished, and the final generated images were selected. We visualize samples from the different target training sets in \cref{fig:dataset_samples}. 

We also computed the FID scores between the different datasets used to train the StyleGAN2 and target models to quantify the visual differences between the datasets and build a baseline for the attacks. Results are stated in \cref{tab:dataset_fid}. We further measured the mean feature distances between the samples of the same class in our datasets. 

We then averaged the results across all classes and stated the results together with the standard deviation in \cref{tab:dataset_dist}. Note that we did not compute the minimum distances between samples to take into account that FaceScrub and CelebA contain samples from the same class that are visually identical and only vary in resolution or cropped image parts. Also, some samples are the horizontally flipped version of another sample. 

\textbf{FaceScrub.} FaceScrub provides cropped face images of 530 identities and is published under the CC BY-NC-ND 3.0 license\footnote{\href{https://creativecommons.org/licenses/by-nc-nd/3.0/}{https://creativecommons.org/licenses/by-nc-nd/3.0/}}. Originally, FaceScrub provided 106,863 samples, but since only links instead of images are provided, we were only able to obtain 37,878 samples. Our train/test split resulted in a total of 34,090 training and 3,788 test samples for FaceScrub. We want to point out that a significant share of FaceScrub samples is mislabelled or of low resolution, which makes learning to classify the images even harder. Also, images of a specific target might strongly vary in style, e.g., showing a person of different ages, with different hair colors, facial accessories, etc. The FaceScrub dataset is available at \href{http://vintage.winklerbros.net/facescrub.html}{http://vintage.winklerbros.net/facescrub.html}.

\textbf{CelebA.} CelebA also contains facial images of celebrities and is available for non-commercial research purposes only. To increase the quality of the CelebA samples, we create a new dataset of cropped and aligned images using the HD CelebA Cropper, available at \href{https://github.com/LynnHo/HD-CelebA-Cropper}{https://github.com/LynnHo/HD-CelebA-Cropper}. We cropped the images using a face factor of 0.65 and resized them to $224\times 224$ using bicubic interpolation. The other parameters were left at default. We then took the 1,000 identities with the most number of samples out of 10,177 available identities. This leaves us with 27,034 training and 3,004 test samples. The total dataset consists of 202,599 images. For comparison, the official CelebA dataset of aligned faces only provides images with a size of $218 \times 178$. The CelebA dataset is available at \href{https://mmlab.ie.cuhk.edu.hk/projects/CelebA.html}{https://mmlab.ie.cuhk.edu.hk/projects/CelebA.html}.

\clearpage
